PanSR: An Object-Centric Mask Transformer for Panoptic Segmentation

Panoptic segmentation is a fundamental task in computer vision and a crucial component for perception in autonomous vehicles. Recent mask-transformer-based methods achieve impressive performance on standard benchmarks but face significant challenges with small objects, crowded scenes and scenes exhibiting a wide range of object scales. We identify several fundamental shortcomings of the current approaches: (i) the query proposal generation process is biased towards larger objects, resulting in missed smaller objects, (ii) initially well-localized queries may drift to other objects, resulting in missed detections, (iii) spatially well-separated instances may be merged into a single mask causing inconsistent and false scene interpretations. To address these issues, we rethink the individual components of the network and its supervision, and propose a novel method for panoptic segmentation PanSR. PanSR effectively mitigates instance merging, enhances small-object detection and increases performance in crowded scenes, delivering a notable +3.4 PQ improvement over state-of-the-art on the challenging LaRS benchmark, while reaching state-of-the-art performance on Cityscapes. The code and models will be publicly available at https://github.com/lojzezust/PanSR.

==> sec/trash/cutout.tex <==
Intro:
----------------------------------------
\section{Introduction}

% Problem 1: Metode nagnjene k detekciji velikih objektov (zaradi top K)
% Problem 2: 
% Problem 3: loss oz. matching je nenaraven (proposali morajo naslavljati objekte, ki niso v proposalih, tekmujejo med sabo)
% 

\begin{figure}[th]
\centering
\includegraphics[width=\linewidth]{figures/cover.pdf}
\caption{Recent transformer-based methods for panoptic segmentation rely on a simple query proposal approach (top left) and struggle with instance separation in predictions (bottom left). Our method utilizes an object-centric query proposal approach (top right) and reworks the mask decoding process for thing classes, leading to significant improvements in instance segmentation (bottom right).}\label{fig:cover}
% \caption{We introduce a robust panoptic method, that addresses the shortcomings of recent transformer-based methods, including proposal drift during decoding (1) and over-segmentation of similar objects (2).}\label{fig:cover}
\end{figure}

Panoptic segmentation is one of the fundamental tasks of computer vision and scene understanding and aims to unify the tasks of semantic segmentation and object detection/instance segmentation. 
Recent trends in this field foster the emergence of transformer-based mask-decoder architectures with the promise of handling different segmentation tasks (segmentation and detection) in a single unified architecture~\cite{Cheng2021Mask2Former,Li2022Mask}.

Mask transformer architectures perform panoptic segmentation through a set of learnable queries, each encoding an individual mask instance. These queries are gradually refined via cross attention with multi-scale image features in the transformer decoder. From the final refined queries, object label, mask and optionally bounding box are predicted. During training, bipartite matching is used for optimal matching between learnable queries and ground-truth instances. This approach leads to great results on general panoptic benchmarks such as COCO~\cite{?} and ADE20k~\cite{?} as well scene parsing in autonomous vehicles  Cityscapes~\cite{?}. However, with the recent release of the LaRS benchmark~\cite{?}, several shortcomings of these approaches were outlined. LaRS focuses on perception of aquatic scenes for autonomous surface vehicles. The visibility range in aquatic scenes is much greater than it's general counterparts, leading to a large range of object sizes, proving difficult for these approaches. 

% Issue 1: proposals fail to addresss objects of different scales
Recent advances in detection capabilities of mask transformers, replacing learnable queries with query selection (\ie proposals) mechanisms~\cite{maskdino,openseed}, improve the robustness of models to different object scales. However, we observe that the simple top-k selection process of these methods is not sufficient to tackle diverse object sizes, as large objects are unfairly favored due to their higher pixel counts, often leading to subpar performance on other objects in the scene (see Figure~\ref{fig:cover}).


\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/problems.pdf}
\caption{Problems of mask transformer methods: query drift after good initialization (top), instance merging of objects (bottom).}\label{fig:problems}
\end{figure}

% Issue 2: query drift. Potrebno skrajšati
In addition, with the introduction of query proposals, other details of the network haven't been reworked in a synergetic way. For example, bipartite matching meshes well with proposals, encouraging the decoding of matched queries towards the corresponding ground-truth, while pushing un-matched queries away. 
%This meshes well with the learnable nature of queries and the behaviour of individual queries targeting different areas in the image naturally emerges as a result~\cite{Cheng2021Mask2Former}. 
However, in the case of query selection the proposals have an associated initial position. In the case of multiple proposals on the same objects, the redundant queries might match to a different object. While this does improve the training objective function, it can lead to unpredictable behavior during inference. In practice this often manifests as \textit{query drift}, where good initial queries drift away from the object during the decoding, even in the absence of alternative queries for the object (Figure~\ref{fig:problems}).
% TODO: drug primer je več proposalov na objekt. V tem primeru želimo, da se vse alternativne hipoteze dekodirajo v isti objekt, ne da tekmujejo med sabo.

% Issue 3: over segmentation (ravnokar izvedel, da je to v resnici undersegmentation, tako da mogoče bolje najti boljši izraz).
% Issue 3: instance merging
Furthermore, the approach for predicting the final instance mask remains largely the same -- a simple dot product operation between the query and high-resolution mask features. As a consequence, to separate instances well, mask features need to learn to encode strong instance information. Despite this, instance merging is common, where predicted masks contain parts of other similar objects in the scene (Figure~\ref{fig:problems}), even when bounding boxes are correctly localized. This is especially common in densely populated scenes.

% Our method PanSR
To address these fundamental issues we propose \method{}, a new scale-robust mask-transformer method for panoptic segmentation, which is our primary contribution. \textbf{1)} To capture objects at all scales, we introduce an object-centric proposal module (OCP), which shifts proposal extraction from pixel-level to object-level and improves performance on small objects. \textbf{2)} To prevent query drift, we introduce a new proposal-aware matching scheme, which prevents matching of proposals to wrong ground-truth instances and allows multiple proposals to match to the same ground-truth instance. This removes the competition between proposals of the same object and instead encourages them to decode alternative predictions for the same object. \textbf{3)} Finally, to address the problem of instance merging, we introduce object-centric mask prediction, where we use the predicted bounding box to constrain the mask prediction to a local area. This removes the requirement of learning strong global instance separation features and frees up the network capacity for other tasks. \textbf{4)} Additionally, to improve robustness to variance in the query selection process, we introduce a set of mask-conditioned queries during training, by sampling queries from random locations in object regions.

% TODO: 

\begin{figure*}[th]
\centering
\includegraphics[width=0.8\textwidth]{figures/architecture_main.pdf}
\caption{Architecture of \method{}. Features extracted by the backbone are processed with a transformer encoder to form a feature pyramid. Object-Centric Proposal extractor (OCP) is used to obtain thing queries. A transformer decoder is used to refine the instance queries. For thing classes we limit the segmentation prediction to a local area predicted by the bounding box. We also employ a new one-to-many matching scheme to increase the stability and robustness of the decoder.}\label{fig:architecture}
\end{figure*}


We evaluate PanSR on LaRS~\cite{Zust2023LaRS}, a recent diverse and challenging aquatic scene parsing benchmark, where it outperforms all existing methods by a large margin (+3.4\% PQ), and on Cityscapes~\cite{?}, where it performs on par with related state-of-the-art methods (67.3 PQ). Ablation study of the major components of our approach demonstrates a large impact of all our major contributions. Additionally, quantitative and qualitative analysis reveals superior performance on small objects, in dense scenes, and in scenes with many similar objects.

%, as well as increased stability of the decoding process and a more evenly distributed spread of proposals across different scales.
% TODO: Combining into a network, experiments, results

% TODO: Summary of contributions

% However, the efforts to merge the different tasks largely ignore the fundamental differences between these tasks and need to make trade-offs in unified architecture choices that favour one task over the other. For example, ~\cite{Cheng2021Mask2Former} uses learnable queries, which have been shown to perform poorly on small objects and scenes with large number of object instances~\cite{?}. On the other hand, some methods~\cite{Li2022Mask} tackle this issue by utilizing dynamic query selection for all its queries, effectively boosting the detection of thing instances. However, the query selection process relies on the selection of salient (je to prava beseda?) features to identify queries for object instances, and thus does not perform well for the segmentation of non-salient stuff (background) classes such as sky and water.

% In this work, we reconsider these choices and unify the benefits of both approaches. Specifically, we consider the unique aspects of stuff and things and make careful design choices that reflect them. First, we investigate query initialization. 


% To summarize, our contributions may be summarized as follows: 1) Query initialization -- we use learnable queries for stuff queries and query selection (i.e. proposals) for thing queries, 2) Object-centric proposals -- we utilize an object-centric approach to proposal generation, that aims to produce a single unique proposal per-object, regardless of object size, 3) Object-centric segmentation -- thing instance segmentation is only responsible for segmenting the object inside its local region determined by the predicted bounding box, and 4) Multi-instance matching -- we improve the matching procedure by filtering out poor matches and allowing multiple matches per single GT. 

% Our method disentangles the queries into queries for background classes (stuff) and foreground instances (things). These two tasks have completely different characteristics. Background segmentation is closely related to semantic segmentation, with the goal of classifying pixels into a fixed set of categories. Foreground instance segmentation is more closely related to detection with the goal of localizing and segmenting instances of objects. These fundamental differences are largely ignored by recent methods. For example Mask2Former conditions its mask predictions on a fixed set of learnable queries and is more suitable for semantic segmentation, while Mask DINO initializes all its queries with a query selection process, which is more suited for detecting foreground objects. Our method combines the benefits of both approaches and also considers the differences in other aspects of the design.

% Selling points
% - Small objects, large numbers of objects -> proposals are the way to go
% - But: How to generate proposals smartly? Existing methods just select top K class logit responses
% - 
-----------------------------------------
